Adaptive Cross-Packet HARQ

In this work, we investigate a coding strategy devised to increase the throughput in hybrid ARQ (HARQ) transmission over block fading channel. In our approach, the transmitter jointly encodes a variable number of bits for each round of HARQ. The parameters (rates) of this joint coding can vary and may be based on the negative acknowledgment (NACK) provided by the receiver or, on the past (outdated) information about the channel states. These new degrees of freedom allow us to improve the match between the codebook and the channel states experienced by the receiver. The results indicate that significant gains can be obtained using the proposed coding strategy, particularly notable when the conventional HARQ fails to offer throughput improvement even if the number of transmission rounds is increased. The new cross-packet HARQ is also implemented using turbo codes where we show that the theoretically predicted throughput gains materialize in practice, and we discuss the implementation challenges.

==> figures/Fig.HARQ.Turbo.tex <==
%!TEX root =  ../HARQ.joint.codec.tex
\usetikzlibrary{arrows}
\usetikzlibrary{shapes}
\usetikzlibrary{positioning}
\usetikzlibrary{calc}
\usetikzlibrary{shapes.misc}
\begin{figure}[h]
\begin{center}
\input{./figures/Encoder_model.tex}
\caption{Turbo Codec structure $\Phi_{[k]}$ as the parallel concatenation of $\Phi_{1},...,\Phi_{k}$, where $\pi_1,\ld\pi_{2k}$ are random interleaver feeding convolutional codes $enc_1,...enc_{2k}$. The structure is used for decoding of 2 transmissions carrying sequences $m_1$ and $m_2$ being jointly encoded.}\label{Fig.HARQ,Turbo}
\end{center}
\end{figure}

